Acoustic disguising: a unified framework for cloaking and holography

Cloaking and holography -- usually treated as distinct problems -- are two limits of a single operation that we call acoustic disguising, realized here using immersive boundary conditions on a closed surface. Driving the boundary with homogeneous Green's functions suppresses any incident field inside the enclosed volume and cloaks unknown objects broadband; driving it with scattering Green's functions synthesizes a holographic scatterer indistinguishable from a target for arbitrary illuminations. Combining the two, using heterogeneous Green's functions, replaces the scattering signature of one object with that of another, transforming its acoustic identity. We demonstrate the framework in three-dimensional FDTD simulations driven by impulsive Green's functions, complemented by data-driven Green's-function retrieval, establishing a direct route to real-time 3D acoustic cloaking, holography, cloning, and disguising.

==> fig/sim/gf/hom-sphere_p_pin_mdd.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{0.5}%
\def\jpgVmax{1.266e+09}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{hom-sphere}%
\def\jpgField{p_pin}%
\def\jpgSource{mdd}%
\def\jpgInnerIdx{0}%
\def\jpgSortBy{dist_outer_to_inner}%
\def\jpgTimePixels{2000}%
\def\jpgAlpha{3.24e-05}%


==> fig/sim/gf/hom-sphere_p_pin_ref.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{0.5}%
\def\jpgVmax{1.266e+09}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{hom-sphere}%
\def\jpgField{p_pin}%
\def\jpgSource{ref}%
\def\jpgInnerIdx{0}%
\def\jpgSortBy{dist_outer_to_inner}%
\def\jpgTimePixels{2000}%
\def\jpgAlpha{1}%


==> fig/sim/gf/hom-sphere_v_pin_mdd.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{0.5}%
\def\jpgVmax{708.7}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{hom-sphere}%
\def\jpgField{v_pin}%
\def\jpgSource{mdd}%
\def\jpgInnerIdx{0}%
\def\jpgSortBy{dist_outer_to_inner}%
\def\jpgTimePixels{2000}%
\def\jpgAlpha{3.037e-05}%


==> fig/sim/gf/hom-sphere_v_pin_ref.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{0.5}%
\def\jpgVmax{708.7}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{hom-sphere}%
\def\jpgField{v_pin}%
\def\jpgSource{ref}%
\def\jpgInnerIdx{0}%
\def\jpgSortBy{dist_outer_to_inner}%
\def\jpgTimePixels{2000}%
\def\jpgAlpha{1}%


==> fig/sim/gf/hom_p_pin_mdd.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{0.5}%
\def\jpgVmax{1.266e+09}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{hom}%
\def\jpgField{p_pin}%
\def\jpgSource{mdd}%
\def\jpgInnerIdx{0}%
\def\jpgSortBy{dist_outer_to_inner}%
\def\jpgTimePixels{2000}%
\def\jpgAlpha{3.24e-05}%


==> fig/sim/gf/hom_p_pin_ref.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{0.5}%
\def\jpgVmax{1.266e+09}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{hom}%
\def\jpgField{p_pin}%
\def\jpgSource{ref}%
\def\jpgInnerIdx{0}%
\def\jpgSortBy{dist_outer_to_inner}%
\def\jpgTimePixels{2000}%
\def\jpgAlpha{1}%


==> fig/sim/gf/hom_v_pin_mdd.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{0.5}%
\def\jpgVmax{708.7}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{hom}%
\def\jpgField{v_pin}%
\def\jpgSource{mdd}%
\def\jpgInnerIdx{0}%
\def\jpgSortBy{dist_outer_to_inner}%
\def\jpgTimePixels{2000}%
\def\jpgAlpha{3.037e-05}%


==> fig/sim/gf/hom_v_pin_ref.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{0.5}%
\def\jpgVmax{708.7}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{hom}%
\def\jpgField{v_pin}%
\def\jpgSource{ref}%
\def\jpgInnerIdx{0}%
\def\jpgSortBy{dist_outer_to_inner}%
\def\jpgTimePixels{2000}%
\def\jpgAlpha{1}%


==> fig/sim/gf/sphere_p_pin_mdd.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{0.5}%
\def\jpgVmax{1.266e+09}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{sphere}%
\def\jpgField{p_pin}%
\def\jpgSource{mdd}%
\def\jpgInnerIdx{0}%
\def\jpgSortBy{dist_outer_to_inner}%
\def\jpgTimePixels{2000}%
\def\jpgAlpha{3.24e-05}%


==> fig/sim/gf/sphere_p_pin_ref.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{0.5}%
\def\jpgVmax{1.266e+09}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{sphere}%
\def\jpgField{p_pin}%
\def\jpgSource{ref}%
\def\jpgInnerIdx{0}%
\def\jpgSortBy{dist_outer_to_inner}%
\def\jpgTimePixels{2000}%
\def\jpgAlpha{1}%


==> fig/sim/gf/sphere_v_pin_mdd.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{0.5}%
\def\jpgVmax{708.7}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{sphere}%
\def\jpgField{v_pin}%
\def\jpgSource{mdd}%
\def\jpgInnerIdx{0}%
\def\jpgSortBy{dist_outer_to_inner}%
\def\jpgTimePixels{2000}%
\def\jpgAlpha{3.037e-05}%


==> fig/sim/gf/sphere_v_pin_ref.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{0.5}%
\def\jpgVmax{708.7}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{sphere}%
\def\jpgField{v_pin}%
\def\jpgSource{ref}%
\def\jpgInnerIdx{0}%
\def\jpgSortBy{dist_outer_to_inner}%
\def\jpgTimePixels{2000}%
\def\jpgAlpha{1}%


==> fig/sim/gf_sphere.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{2.983}%
\def\jpgVmax{3.021e+04}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{sphere}%
\def\jpgInnerIdx{0}%
\def\jpgField{GF_p_q}%
\def\jpgSortBy{dist_outer_to_inner}%
\def\jpgTimePixels{16000}%


==> fig/sim/inner_sphere.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{30}%
\def\jpgVmax{4.705}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{sphere}%
\def\jpgIllIdx{231}%
\def\jpgField{p}%
\def\jpgSortBy{dist_inner_to_ill}%
\def\jpgTimePixels{16000}%


==> fig/sim/outer_sphere.meta.tex <==
% auto-generated by figures/preprocess/_jpg_panel.py — do not edit
\def\jpgXmin{1}%
\def\jpgXmax{400}%
\def\jpgYmin{0}%
\def\jpgYmax{30}%
\def\jpgVmax{1.928e-06}%
\def\jpgCmap{crameri:vik}%
\def\jpgScatterer{sphere}%
\def\jpgIllIdx{231}%
\def\jpgField{v_in}%
\def\jpgSeparation{normal_incidence}%
\def\jpgSortBy{dist_outer_to_ill}%
\def\jpgTimePixels{16000}%

